Certification of Iterative Predictions in Bayesian Neural Networks

We consider the problem of computing reach-avoid probabilities for iterative predictions made with Bayesian neural network (BNN) models. Specifically, we leverage bound propagation techniques and backward recursion to compute lower bounds for the probability that trajectories of the BNN model reach a given set of states while avoiding a set of unsafe states. We use the lower bounds in the context of control and reinforcement learning to provide safety certification for given control policies, as well as to synthesize control policies that improve the certification bounds. On a set of benchmarks, we demonstrate that our framework can be employed to certify policies over BNNs predictions for problems of more than $10$ dimensions, and to effectively synthesize policies that significantly increase the lower bound on the satisfaction probability.

==> Sections/Methodology.tex <==
\section{Probabilistic Reach-Avoid Computation }
\label{sec:ReachAvoid}
% In this section f

\iffalse

For compact sets $X_{k},X_{k+1}\subset \mathbb{R}^m$ and $u\in \mathcal{U}$ we first show how to compute a non-trivial lower bound for 
% $\inf_{x\in X}T^{}(\bar{X}|{x})$
$\inf_{x\in X_k}T^{}(X_{k+1}|{x},u)$ \np{it should be $\inf_{x\in X_k}T^{}(X_{k+1}|{x}, \pi(x))$, right?}\LL{Yep}, that is, 
% \ref{sec:SingleStep} for compact sets $X_1,X_2\subset \mathbb{R}^m$ we show how to compute $\min_{x\in X_1}T^{}(X_2|{x}), \max_{x\in X_1}T^{}(X_2|{x})$, that is 
% the minimum of the one-step transition probabilities of a BNN, given any of the starting points in a compact set. 
% the minimum one-step transition probability of the BNN, given any of the starting points in a compact set. 
the minimum one-step probability of reaching a state in $X_{k+1}$  from any state in $X_{k}$. 
Thereafter, we show how these quantities can be propagated over time to compute a lower-bound for $P_{reach}$ via a backward iterative procedure.

\subsection{Worst-Case Single Step Bounds? }
\label{sec:SingleStep}

As discussed above, in order to solve Problem \ref{Prob:verification}  we first need to find a non-trivial lower bound for
\begin{align}
    \label{Eqn:singleStep}
    % \inf_{x\in X}T^{}(\bar{X}|{x}) 
    \inf_{x\in X_k}T^{}(X_{k+1}|{x},u) 
\end{align}
for compact sets 
% $X,\bar{X}\subset \mathbb{R}^m$.
$X_k,X_{k+1}\subset \mathbb{R}^m$. 
Such quantities give the ranges of the probability that the BNN output lies in 
% $\bar{X}$, given any of the input points $x\in X$. 
$X_{k+1}$, given any of the input points $x\in X_k$. 
% This single step probabilities will then be propagated over time in the next Section. 
However, the computation of Eqn \eqref{Eqn:singleStep} is not trivial as the distribution of $f^{\mathbf{v}}(x)$ is intractable in general and even the exact computation of 
non-probabilistic reachability for deterministic NNs is a hard problem that cannot be solved in practice for state-of-the-art neural networks \cite{}. \np{I removed the NP thing, because I believe it is more complex than NP (e.g., Reluplex uses a combination of SMT+simplex, and simplex is already exp-time, and moreover it works only for PW-linear activations)}

% these ranges for a deterministic NN is an NP problem, which cannot be solved in practice for state-of-the-art neural networks  \cite{}. 
However, we can rely on recent results in the context of constraint relaxations for BNNs to find upper and lower bounds for these quantities \cite{wicker2020probabilistic}.

\LL{HERE WRITE IBP THEOREM, basically a condesed version of Proposition 1 and Section 4.1 in the UAI paper. I leave this to Andrea}

\LL{Note that Eqn \eqref{Eqn:singleStep} can be lower bounded with our UAI method as per Proposition 4 in the supplementary. }

\subsection{Backward Computation of  Probabilistic Reach-Avoid}
We show how to compute a lower bound of $P_{reach}$ through a backward iterative procedure.
A backward approach is particularly suited in this setting to synthesize robust strategies via dynamic programming \cite{} and to account for the BNN uncertainty by employing Theorem \ref{}.
%For many applications the uncertainty in the BNN predictions can be large because of the large number of parameters in the BNN and/or of the avaiability of only few data points to train the BNN. As a consequence, simply propagating forward over time this uncertainty can lead to very uncertain dynamics after just few steps. This is illustrated in Figure \ref{fig:step2} for a two dimensional problem. 
%\LL{We need to discuss why we do backward instead of forward. I mean, backward is surely better to be extended for synthesis in the case of discrete controllers (that we should), but we need also to explain why forward would not give nice probabilities.} \LL{The algorithm is that it can be conservative. So, we need to explain why this is still good when combined with UAI}\acmt{Can we justify this computation in view of the model-based DP analogue recursions, which are precursors to the Bellman iterations for strategy synthesis?} 

For a time interval $[0,N]$ and a function $\beta:\mathbb{R}^n\times [0,N]\to \mathcal{B}(\mathcal{G}\cup \mathcal{S})$, that assigns a Borel set of points that are either safe or in the goal region for any pair (state,time),  consider the set of functions $V_k^{\pi,\beta}:\mathbb{R}^n\to [0,1]$ defined with the following backward recursion for $0\leq k<N$ \LL{Need some updates about the $\beta$ functions to check this is exactly what is implmented in the code}
\np{not clear to me what's the role of $\beta$, how you define it}
\begin{align}
    &\nonumber V_N^{\pi,\beta}(x)=\mathbf{1}_\mathcal{G}(x) \\
    &V_k^{\pi,\beta}(x)= T({\beta({x},k})|x,\pi({x},k)) \cdot \inf_{\bar x \in \beta({x},k)} V_{k+1}^{\pi,\beta}(\bar x).% \\
   % &{\color{blue}\int_{\bar{x} \in\beta(x,k)} T^{} (\bar{x} \mid x) \cdot V^{\pi}_{k+1}(\bar{x})d \bar{x}} 
    \label{Eqn:ValueFunc}
\end{align}
\np{equation above should be $V_k^{\pi,\beta}(x)= T({\beta({x},k})|x,\pi(x)) \cdot \inf_{\bar x \in \beta({x},k)} V_{k+1}^{\pi,\beta}(\bar x)$, right? (policy does not depend on time)}\LL{Policy does depend on time. This is because the optimal policy for reach avoid specifications are time-dependent. I mean, if we want we can drop the time dependence, but we cannot guarantee we will have an optimal strategy for the specification. In any case, I am not super satisfied with this formulation, as these beta functions look a bit cumbersome.}
\np{I agree that the synthesized policy depends on time. then, we should clarify the difference with the $\pi$ used in (1)}
Intuitively, for any state $x$ and time index $k$, $\beta({x},k)$ is a set of states such that if System \eqref{Eqn:SystemEqn} starts from each of those states at time $k+1$, it will have high probability of satisfying the reach-avoid specification (note that Eqn \eqref{Eqn:ValueFunc} is solved backward, hence such a set of states can be easily computed)  and such that starting from $x$ the BNN will have high probability of reaching those at the following time step. An algorithm detailing how to compute $\beta$ will be given in Section \ref{sec:Algorithm}. 
The following theorem guarantees that for any function $\beta$ the solution of the above backward recursion is a lower bound for $P_{reach}(\mathcal{G},\mathcal{S},x,[k,N]|\pi).$



\begin{theorem}
\label{th:CorrectnessBack}
Assume, as per Problem 1, that $\mathcal{G}\cap \mathcal{S}=\emptyset$. Then, for any $k\leq N$, function $\beta,$ and strategy $\pi$ it holds that
$$  P_{reach}(\mathcal{G},\mathcal{S},x,[k,N]|\pi)\geq  V_k^{\pi,\beta}(x).$$
\end{theorem}
\begin{proof}
The proof is by induction. The base case is $k=N$, for which we have
$$V_N^{\pi,\beta}(x) \leq P_{reach}(\mathcal{G},\mathcal{S},x,[N,N]|\pi)= \mathbf{1}_\mathcal{G}(x), $$
which is trivially verified. Now with the assumption that for any $k\in \{0,N-1 \}$ it holds that \np{$q$ below is not introduced before}
\begin{align}
    \label{Eqn:IndBaseCase}
    \inf_{x\in {\beta({x},k})} V_{k+1}^{\pi,\beta}(x) \leq \inf_{x\in {\beta({x},k})}P_{reach}(\mathcal{G},\mathcal{S},x,[k+1,N]|\pi),
\end{align}
we can show the induction step.
In particular, for any $x$ the following holds (in the rest of the proof for simplicity we omit the dependence of the strategy from $Pr$):
\begin{align*}
     &P_{reach}(\mathcal{G},\mathcal{S},x,[k,N]|\pi)=\\
     &\sum_{j=k+1}^{N}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' < j, \omega(j') \in \mathcal{S} |\omega(k)= x)\geq\\
    &Pr( \omega(k+1) \in \mathcal{G} |\omega(k)= x ) +\\
    &\quad Pr( \omega(k+1) \in (\beta(x,k)-\mathcal{G}) |\omega(k)= x ) \sum_{j=k+2}^{N}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' < j, \omega(j') \in \mathcal{S} |\omega(k+1)\in (\beta(x,k)-\mathcal{G}))\geq\\
    &Pr( \omega(k+1) \in\beta(x,k) |\omega(k)= x ) \sum_{j=k+2}^{N}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' < j, \omega(j') \in \mathcal{S} |\omega(k+1)\in (\beta(x,k)-\mathcal{G}))\geq\\
    &Pr( \omega(k+1) \in\beta(x,k) |\omega(k)= x )\inf_{\bar x \in\beta(x,k)} \sum_{j=k+2}^{N}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' < j, \omega(j') \in \mathcal{S} |\omega(k+1)=\bar x)=\\
    &T^{}(\beta(x,k)|x)\inf_{\bar x \in\beta(x,k)} P_{reach}(\mathcal{G},\mathcal{S},\bar x,[k+1,N])\geq \\
    &T^{}(\beta(x,k)|x)\cdot \inf_{\bar x \in\beta(x,k)} V_{k+1}^{\pi,\beta}(\bar x)= V_k^{\pi,\beta}( x),
\end{align*}
where the third step of the proof holds because  $\sum_{j=k+2}^{N}P( \omega(j) \in \mathcal{G} \wedge \forall j' < j, \omega(j') \in \mathcal{S} |\omega(k+1)\in (\beta(x,k)-\mathcal{G}))$ is a sum of the probabilities of mutually exclusive events, hence a probability itself and by definition smaller or equal than $1$. 
\end{proof}
\begin{corollary}
Under the same assumptions of Theorem \ref{th:CorrectnessBack}, for any $k\leq N$, function $\beta,$ and strategy $\pi$ it holds that
$$  P_{reach}(\mathcal{G},\mathcal{S},x,[0,N]|\pi)\geq  V_k^{\pi,\beta}(x).$$
\end{corollary}
\begin{proof}
The statement holds by simply noticing that
$P_{reach}(\mathcal{G},\mathcal{S},x,[0,N])\geq P_{reach}(\mathcal{G},\mathcal{S},x,[0,k])= P_{reach}(\mathcal{G},\mathcal{S},x,[N-k,N]).$
\LL{This may not be true if the strategy depends on the full history, but for the strategies considered in here this holds.}
\end{proof}


$V_k^{\pi,\beta}$, as computed in Eqn \eqref{Eqn:ValueFunc}, is a formal lower bound of $P_{reach}$ for any $\beta$ such that $\beta(x,k)\subseteq  \mathcal{G}\cup \mathcal{S}$. However, the choice of $\beta$ has a great effect on the resulting lower bound. For instance, in order to have non-zero lower bound it is required that  $\beta(x,N)\subseteq  \mathcal{G}$ for any $x$. A possible choice of this function to maximize the lower bound is described in the next Section and implemented in Algorithm \ref{}. However, before of discussing the algorithm, in the following remark, we highlight the rationale behind our approach in the computation of $P_{reach}.$


\begin{remark}
$V_k^{\pi,\beta}$, as computed with Eqn \eqref{Eqn:ValueFunc}, is a formal lower bound for $P_{reach}$. A question that may arise is why we decide to consider a lower bound instead of the exact quantity. In order to illustrate this point we can consider the following set of functions $\bar{V}_k^{\pi}:\mathbb{R}^n\to [0,1]$ defined with the following backward recursion for $0\leq k<N$
\begin{align}
    &\nonumber \bar{V}_N^{\pi}(x)=\mathbf{1}_\mathcal{G}(x) \\
    &\bar{V}_k^{\pi}(x)=\mathbf{1}_\mathcal{G}(x)+\mathbf{1}_\mathcal{S}(x){\int T^{} (\bar{x} \mid x) \cdot \bar{V}^{\pi}_{k+1}(\bar{x})d \bar{x}}, %=\mathbf{1}_\mathcal{G}(x)+\mathbf{1}_\mathcal{S}(x)\mathbb{E}_{T^{} (\bar{x} \mid x)}[ \bar{V}^{\pi}_{k+1}(\bar{x})]
    \label{Eqn:ExactValueFunc}
\end{align}
where with an abuse of notation $T^{} (\bar{x} \mid x)$ is the pdf of the stochastic kernel induced by the BNN.
It is easy to realize that $P_{reach}(\mathcal{G},\mathcal{S},x,[0,N])=\bar{V}_0^{\pi}(x)$. However, unfortunately, computation of Eqn \eqref{Eqn:ValueFunc} requires the computation of a multidimensional integral over the BNN distribution, which is infeasible \cite{blaas2020adversarial}. In Eqn \ref{Eqn:ValueFunc} we solve this issue by considering a lower bound that can be easily computed and that can also be efficiently optimized as described in Section \ref{Sec:Syntesis}. \end{remark}



\fi

\LL{Alternative presentation could be do first introduce the exact backward eqautions for $P_{reach}$ (Eqn 5) and then introduce directly $K$ in the next section without introducing Eqn 4. Presentation will be probably clearer. So, if you agree, I will do that. }


We show how to compute a lower bound of $P_{reach}$ through a backward iterative procedure.
A backward approach is particularly suited in this setting to propagate the uncertainty of the neural network and also to synthesize robust strategies via dynamic programming, as we will show in the next Section.
To this purpose,  for a time interval $[0,N]$ and a partition of $[0,1]$ in $n_p$ intervals $0=v_0< v_1<...<v_{n_p}=1$, consider the set of functions $V_k^{\pi}:\mathbb{R}^n\to [0,1]$ defined with the following backward recursion for $0\leq k<N$ 
\begin{align}
    &\nonumber V_N^{\pi}(x)=\mathbf{1}_\mathcal{G}(x) \\
    &V_k^{\pi}(x)= \mathbf{1}_\mathcal{G}(x) + \mathbf{1}_\mathcal{S}(x) \sum_{i=1}^{n_p}v_{i-1}\int_{H^{x}_{k,i}}p_{\mathbf{v}}(v|\mathcal{D})   dv,% \\
   % &{\color{blue}\int_{\bar{x} \in\beta(x,k)} T^{} (\bar{x} \mid x) \cdot V^{\pi}_{k+1}(\bar{x})d \bar{x}} 
    \label{Eqn:ValueFunc}
\end{align}
\acmt{I would recommend clarifying more at length the terms $v_{k,i}^{L}$ and $v_k^{U}$}\LL{100\%. Doing it now}
where $H_{k,i}^x=\{ w \, : \, v_{i-1}\leq V_{k+1}^{\pi}(f^w(x,\pi(x,k))) \leq v_{i}  \}$. %and such that for each  $k\in [0,N],$ $H_{k,i}^x \cap H_{k,j}^x=\emptyset $ for $i,j\in \{1,...,n_p \}$.
Intuitively, sets $H_{k,i}^{x}$ partition the weight space of the BNN according to the values of the value function at the next time step (note that $0\leq V_{k+1}^{\pi} \leq 1$). Note that sets of weights $H_{k,i}^{x}$ and $H_{k,j}^{x}$ for $i\neq j$ are overlapping for sets of at most measure zero.  

We should stress that Eqn \eqref{Eqn:ValueFunc} is solved backward. In fact, the partitioning of the weight space is done backward based on the value function at the next time-step.
The following theorem guarantees that the solution of the above backward recursion is a lower bound for $P_{reach}(\mathcal{G},\mathcal{S},x,[k,N]|\pi).$ \LL{Actually, we have convergence. So, we may want to highlight that in Theorem 1}



\begin{theorem}
\label{th:CorrectnessBack}
Assume, as per Problem 1, that $\mathcal{G}\cap \mathcal{S}=\emptyset$. Then, for any $k\leq N$ it holds that
$$  P_{reach}(\mathcal{G},\mathcal{S},x,[k,N]|\pi)\geq  V_k^{\pi}(x).$$
\end{theorem}
\begin{proof}
Proof is commented in here.
\end{proof}

\begin{corollary}
Consider the same assumptions of Theorem \ref{th:CorrectnessBack} and further assume that $\pi$ is stationary, i.e., for any $x\in \mathbb{R}^{n}$ $k_1,k_2\leq N$ we have that $\pi(x,k_1)=\pi(x,k_2)$, then for any $k\leq N$ it holds that
$$  P_{reach}(\mathcal{G},\mathcal{S},x,[0,N]|\pi)\geq  V_k^{\pi}(x).$$
\end{corollary}
\begin{proof}
The statement holds by simply noticing that
$P_{reach}(\mathcal{G},\mathcal{S},x,[0,N])\geq P_{reach}(\mathcal{G},\mathcal{S},x,[0,k])= P_{reach}(\mathcal{G},\mathcal{S},x,[N-k,N]).$ 
\acmt{Are we sure about this statement? It would seem reasonable for a `reach' specification, but does it still hold in general if there is an avoid set? (what if the dynamics `leak' towards the avoid set more than they get `attracted' to the reach one?) ((also, pls clarify/remind function beta in statement.))}\LL{It should work due to the fact that the dynamics are Markovian, we start from the same fixed initial state, and the strategy is stationary, which is not the case anymore in the new prob formulation. So, I have added this further assumption.}\LL{Also, we do not really use this Corollary in the paper, so it can even be removed without any problem.}
\end{proof}

While the backward recursion in Eqn \eqref{Eqn:ValueFunc} may seem rather complex to be solved. In the next Sections we show how this can be formally and efficiently computed (Section \ref{sec:Algorithm}) and also how a strategy that optimize (a lower bound of) $V_k^{\pi}$ can be derived (Section \ref{Sec:Syntesis}). However, before of doing so, we consider two remarks on $V_k^{\pi}$.


\begin{remark}
\LL{Here add formulae for when $p_{\mathbf{v}}(v|\mathcal{D})$ is Gaussian and cite \cite{blundell2015weight}. Everything becomes analytic in this case}
\end{remark}


\begin{remark}
$V_k^{\pi}$, as computed with Eqn \eqref{Eqn:ValueFunc}, is a formal lower bound for $P_{reach}$. A question that may arise is why we decide to consider a lower bound instead of the exact quantity. In order to illustrate this point we can consider the following set of functions $\bar{V}_k^{\pi}:\mathbb{R}^n\to [0,1]$ defined with the following backward recursion for $0\leq k<N$
\begin{align}
    &\nonumber \bar{V}_N^{\pi}(x)=\mathbf{1}_\mathcal{G}(x) \\
    &\bar{V}_k^{\pi}(x)=\mathbf{1}_\mathcal{G}(x)+\mathbf{1}_\mathcal{S}(x){\int T^{} (\bar{x} \mid x, \pi(x,k)) \cdot \bar{V}^{\pi}_{k+1}(\bar{x})d \bar{x}}, %=\mathbf{1}_\mathcal{G}(x)+\mathbf{1}_\mathcal{S}(x)\mathbb{E}_{T^{} (\bar{x} \mid x)}[ \bar{V}^{\pi}_{k+1}(\bar{x})]
    \label{Eqn:ExactValueFunc}
\end{align}
where with an abuse of notation $T^{} (\bar{x} \mid x)$ is the pdf of the stochastic kernel induced by the BNN.
It is easy to realize that $P_{reach}(\mathcal{G},\mathcal{S},x,[0,N])=\bar{V}_0^{\pi}(x)$. However, unfortunately, computation of Eqn \eqref{Eqn:ValueFunc} requires the computation of a multidimensional integral over the distribution of the functions sampled from the BNN, which is infeasible \cite{blaas2020adversarial}. In Eqn \ref{Eqn:ValueFunc} we solve this issue by expressing the multidimensional integral over the space of weights of the BNN (note that the stochastic kernel $T$ is induced by the posterior distribution $p_{\mathbf{v}}(v|\mathcal{D})$) and then we  partition the weight space based on the value function. As we will show in the next Section, this formulation leads to dynamic programming equations that can be formally solved and optimized.


%considering a lower bound that can be easily computed and that can also be efficiently optimized as described in Section \ref{Sec:Syntesis}. 

%Highlight weight against function space


\end{remark}









\subsection{A Formal  Numerical Approach for Computation of $P_{reach}$}
\label{sec:Algorithm}



Even in the case where $p_{\mathbf{v}}(v|\mathcal{D})$  is Gaussian, the computation of $V_{0}^{\pi}$ cannot be performed exactly. In what follows we develop a formal approach based on discretization of the state space that returns a safe lower bound of $V_{0}^{\pi}$. In particular, let $Q=\{q_1,...,q_{n_q} \}$ be a partition of the safe set $\mathcal{S}$ and goal region $\mathcal{G}$ in $n_q$ states. Note that $Q$ is not necessarily a discretization of the all dimensions of the state space. In fact, often we only care about the safety of a subset of the dimensions. With some abuse of notation in what follows we will use $q$ to represent both a state in $Q$ and the correspondent region in $\mathcal{S}\cup \mathcal{G},$ the meaning will be clear from the context. We further call $z:\mathbb{R}^n\to Q,$ the function that associates a state in $\mathbb{R}^n$ to the respective abstract state. Now, for a given strategy $\pi$ and a partition of $[0,1]$ in $n_p$ intervals $0=v_0< v_1<...<v_{n_p}=1$,  consider the set of functions $K^{\pi}_k:Q \to [0,1]$ defined recursively as follow for $k\in \{0,...,N-1 \},$
\begin{align}
    \nonumber&K^{\pi}_N(q)=\mathbf{1}_{\mathcal{G}}(q) \\
    &K^{\pi}_k(q)=\mathbf{1}_{\mathcal{G}}(q) + \mathbf{1}_{\mathcal{S}}(q) \sum_{i=1}^{n_p}v_{i-1}\int_{H^{q}_{k,i}}p_{\mathbf{v}}(v|\mathcal{D})   dv,% 
    \label{Eqn:ValueFuncDiscre}
\end{align}
where $\mathbf{1}_{\mathcal{G}}(q)=\inf_{x\in q}\mathbf{1}_{\mathcal{G}}(x)$,  $\mathbf{1}_{\mathcal{S}}(q)=\inf_{x\in q}\mathbf{1}_{\mathcal{S}}(x)$, and  $$H_{k,i}^q=\{ w \, : \, \forall x\in q, \text{ it holds that }  v_{i-1} \leq  K_{k+1}^{\pi}(z(f^w(x,\pi(x,k)))) \leq v_{i}  \}$$ and such that for each  $k\in [0,N],$ $H_{k,i}^q \cap H_{k,j}^q=\emptyset $ for $i,j\in \{1,...,n_p \}$. 
The following proposition guarantees that $K^{\pi}_k$ is a sound numerical approximation of $V^{\pi}_k.$
\begin{proposition}
\label{prop:VerificationLoerBound}
Given $x\in \mathbb{R}^m$, let $q\in Q$ be such that $x\in q$. Assume the the same partition of $[0,1]$ in $n_p$ intervals $0=v_0< v_1<...<v_{n_p}=1$ for both Eqn \eqref{Eqn:ValueFunc} and Eqn \eqref{Eqn:ValueFuncDiscre}. Then, for any  $k\in \{0,...,N\}$ it holds that
$$ V_{k}^{\pi}(x)\geq  K^{\pi}_k(q).$$
\end{proposition}
\LL{Proof can be simplified. I will do it later, once we have all the other proofs written down}
\begin{proof}
First of all note that
\begin{align}
    & \inf_{x\in q} V_k^{\pi}(x)=\\
    &\mathbf{1}_\mathcal{G}(q) + \mathbf{1}_\mathcal{S}(q)  \inf_{x\in q} \sum_{i=1}^{n_p}v_{i-1}\int_{H^{x}_{k,i}}p_{\mathbf{v}}(v|\mathcal{D})   dv \geq \\
    &\mathbf{1}_\mathcal{G}(q) + \mathbf{1}_\mathcal{S}(q)   \sum_{i=1}^{n_p}v_{i-1}  \inf_{x\in q} \int_{H^{x}_{k,i}}p_{\mathbf{v}}(v|\mathcal{D})   dv.
    \label{Eqn:ProofDIscrCorr}
\end{align}
Now, note that for any $i,j$ it holds that $v_{j} > v_{i} $ if $j>i$. Then,  in order to conclude the proof it suffices to notice that for each $i\in \{1,...,n_p\}$ and $x\in q$ it holds that if $w' \in H^{q}_{k,i}$ then there exists $j\geq i$ such that $w'\in H^{x}_{k,j}$. The proof is by induction. The base case is for $k=N-1$, where we have
$$H_{N-1,i}^q=\{ w \, : \, \forall x\in q, \text{ it holds that }  v_{i-1} \leq \mathbf{1}_{\mathcal{G}}(z(f^w(x,\pi(x,N-1)))) \leq v_{i}  \}$$
$$H_{k,i}^x=\{ w \, : \,   v_{i-1} \leq \mathbf{1}_{\mathcal{G}}(f^w(x,\pi(x,N-1))) \leq v_{i}  \}.$$
There are four possible cases
\begin{itemize}
    \item $\mathbf{v_{i-1}\leq 0<1\leq v_{i}}$. In this case $H_{N-1,i}^x= H_{N-1,i}^q=\mathbb{R}^{n_w}$ as both value functions are between $0$ and $1.$
     \item $\mathbf{v_{i-1}\leq 0<v_{i}< 1}$. In this case $H_{N-1,i}^x\subseteq H_{N-1,i}^q$. 
    \item $\mathbf{0<v_{i-1}< v_{i}<1}$. In this case $H_{N-1,i}^q= H_{N-1,i}^x=\emptyset$ as the indicator function can be only $1$ or $0.$
    \item $\mathbf{0<v_{i-1}<1\leq v_{i}}.$ In this case $H_{N-1,i}^q\subseteq H_{N-1,i}^x$.
\end{itemize}
Hence, the statement holds.

Now we can proceed with the induction step for time $k<N-1$ with the assumption that for each $i\in \{1,...,n_p\}$ and $x\in q$ it holds that if $w' \in H^{q}_{k+1,i}$ then there exists $j\geq i$ such that $w'\in H^{x}_{k+1,j}$. Note that by Eqn \eqref{Eqn:ProofDIscrCorr} this assumption implies that 
$$ \inf_{x\in q} V_{k+1}^{\pi}(x)\geq  K_{k+1}^{\pi}(q). $$
This implies that for any $w\in \mathbb{R}^{n_w}$
$$ V_{k+1}^{\pi}(f^w(x,\pi(x,k))) \geq   K_{k+1}^{\pi}(z(f^w(x,\pi(x,k)))),  $$
which concludes the proof.
\end{proof}

Proposition \ref{prop:VerificationLoerBound} guarantees that for any $x$, $K^{\pi}_{0}(z(x))\leq P_{reach}(\mathcal{S},\mathcal{G},[0,N],x).$ However, its computation still requires to compute sets $H_{k,i}^q$. This boils down to compute a set of weights $H$ such that for a given set $\mathcal{O}\subseteq \mathbb{R}^n$ it holds that for any $x\in q$
$$ \forall w\in H, f^{w}(x,\pi(x,k))\in \mathcal{O}, $$
that is, we need to find the set of parameter vectors such that for each of these parameters set $q$ is propagated by the resulting neural network inside set $\mathcal{O}.$
An safe underapproximation of set $H$ can be computed by relying on the following proposition from \cite{wicker2020probabilistic}.
\begin{proposition}{\cite{wicker2020probabilistic}}
\label{Proposition:UAI}
\LL{ADD UAI IN HEre}
\end{proposition}



\iffalse
% \footnote{\np{I guess that we should also say that we have actually 3 partitions, for $\mathcal{S} \setminus \mathcal{G}$, for $\mathcal{G} \setminus \mathcal{S}$ and for $\mathcal{S} \cap \mathcal{G}$, respectively. Agree?} \np{I don't understand much line 6. 1) what's the threshold $th$? 2) if ${Q}^{enl}$ must be a subset of $\mathcal{G}\cup \mathcal{S}$, then such a  ${Q}^{enl}$ may not exist. 3) in practice, here you apply the UAI algorithm to input region $q$, right? we might want to explain better the functioning of the algo in that it uses a backward scheme, but based on a 1-step forward algorithm. Adding a cartoon of the backwards scheme would help as well} \np{we should define a sequence of $\hat P_{\mathcal{G},\mathcal{S},[0.N]}^{\pi}(x)$ functions (or a primed version of it). O/W the assignment in line 8 is ambiguous (RHS contains ``previous'' version of $\hat P_{\mathcal{G},\mathcal{S},[0.N]}^{\pi}(x)$, right?)} }. 

In particular, for simplicity we assume that $\mathcal{G}\cap \mathcal{S}=\emptyset$. \np{$\mathcal{G}\cap \mathcal{S}=\emptyset$ is in problem definition} Furthermore, we assume that the set $\mathcal{G}\cup \mathcal{S}$ is partitioned into a an arbitrary finite set of non-overlapping regions (except for at most sets of measure zero) $Q=\{q_1,...,q_{|Q|}  \}$. We indicate with $q_i, i\in \{1,...,|Q|\}$ both a member of $Q$ and a region in $\mathbb{R}^m$. In Line $1$ we set to $1$ the probability of satisfying the specification to all states in the goal region $\mathcal{G}$. Then, in line $3-13$ we recursively enlarge the goal region over time in order to account for states that have high probability to reach the extended goal region in a single time step. Algorithm \ref{alg:ForLoop} finally returns $\hat P_{\mathcal{G},\mathcal{S},[0.N]}^{\pi}$ such that for all $x\in \mathcal{S}\cup\mathcal{G}$ it holds that $$\hat P_{\mathcal{G},\mathcal{S},[0.N]}^{\pi}(x)\leq P_{\text{reach}}(\mathcal{G},\mathcal{S},x,[0.N],\pi)$$



\begin{algorithm} \footnotesize
\caption{Probabilistic Reach-Avoid Computation}\label{alg:ForLoop}
\textbf{Input:} $\mathcal{S}$ -- safe region,  $\mathcal{G}$ --goal region, $Q$ --- discretization of $\mathcal{S}\cup \mathcal{G}$.  $T$ -- Time Horizon, $th$ -- threshold, $\pi$ -- stationary policy \\
%\MK{$S$ not explicit but used below, also fix line break}
\textbf{Output:} $\hat P_{\mathcal{G},\mathcal{S}[0.N]}^{\pi}$
, a sound lower bound of $P_{\text{reach}}(\mathcal{G},\mathcal{S},x_0,[0.N],\pi)$ for any $x_0 \in \mathcal{S}\cup \mathcal{G}$ \\
\vspace*{-0.35cm}
\begin{algorithmic}[1]
\STATE for all $x \in  \mathcal{G}$ set $\hat P_{\mathcal{G},\mathcal{S},[0.N]}^{\pi}(x) = 1$ and for all $x \in  \mathcal{S}$ inizialize $\hat P_{\mathcal{G},\mathcal{S},[0.N]}^{\pi}(x) = 0$
% bar G is extended goal region
\STATE $k\gets 0, \bar{\mathcal{G}}\gets \mathcal{G}$
\WHILE{$k<N$}
\STATE $\bar{\mathcal{G}}'\gets \bar{\mathcal{G}}$
% 
\FORALL{$q\in \mathcal{S}\setminus \bar{\mathcal{G}}$}
    % extended UAI
    \STATE compute ${Q}^{enl}\subseteq \bar{\mathcal{G}}\cup \mathcal{S} $ such that $\min_{x\in q} T^{}({Q}^{enl}|x)\geq th$ \COMMENT{See  Theorem \ref{}}
    \IF{${Q}^{enl}\subseteq \bar{\mathcal{G}}$}
        % enlarge goal region
        % 
        \STATE for all $x\in q$ set $\hat P_{{\mathcal{G}},\mathcal{S},[0.N]}^{\pi}(x)=\min_{x\in q} T^{}({Q}^{enl}|x)\cdot \inf_{\bar x \in {Q}^{enl}}\hat P_{{\mathcal{G}},\mathcal{S},[0.N]}^{\pi}(\bar x)$
        \STATE $\bar{\mathcal{G}}'\gets \bar{\mathcal{G}}'\cup q$
    \ENDIF
\ENDFOR
    \STATE $k\gets k+1 \quad \bar{\mathcal{G}}\gets \bar{\mathcal{G}}'$
\ENdvHILE
\STATE return $\hat P_{\mathcal{G},\mathcal{S},[0.N]}^{\pi}$
\end{algorithmic}
\end{algorithm}


\fi

%The underlying idea of our approach is that of starting from the goal region $\mathcal{G}$ and then enlarge it over time to account for all the states that have reached the goal region while being safe with high probability up to that time step.


\section{Synthesis}
\label{Sec:Syntesis}

\LL{To be updated with new formulations of the dynamic programming equations}
We now focus on the synthesis problem, which seeks to find a strategy $\pi$ to optimize $ P_{reach}(\mathcal{G},\mathcal{S},x,[0,N]|\pi).$ In particular, in this paper we focus on synthesizing a strategy that maximizes the lower bound of $P_{reach}$ derived in the previous Section. We stress that by maximizing a lower bound we are guaranteed that the true probability is always greater than the lower bound obtained after maximization.
\begin{definition}{(Maximal Safe Strategy)}.
A strategy $\pi^*$ is called maximal safe iff for all $x\in \mathcal{G}\cup\mathcal{S}$ it holds that
$$  V_{0}^{\pi^*}(x)=\sup_{\pi} V_{0}^{\pi}(x). $$
\end{definition}
%\LL{We may also want to show explicitly that such a policy extsts, even tho may not be needed for the conference version. It should suffice the set of admissible controls is a compact set }
\noindent
Note that such a maximal safe strategy is guaranteed to exist under mild assumptions generally verified in practice. For instance, for the setting in this paper a sufficient condition is that the set of admissible controls $\mathcal{U}$ is compact \cite[Lemma 3.1]{bertsekas2004stochastic}.
In the next theorem we show that a maximal safe strategy can be computed via dynamic programming with a backward recursion similar to that of Eqn \eqref{Eqn:ValueFunc}.
\begin{theorem}
\label{Th:Syntesis}
For for $0\leq k<N$, define $V^*_{k}:\mathbb{R}^n\to [0,1]$  recursively as follows
\begin{align*}
    &V^*_{k}(x)=\sup_{u\in \mathcal{U}} \big( \mathbf{1}_\mathcal{G}(x) + \mathbf{1}_\mathcal{S}(x) \sum_{i=1}^{n_p}v_{k,i}^{L}\int_{H^{x}_{k,i}}p_{\mathbf{v}}(v|\mathcal{D})   dv \big), 
\end{align*}
where $H_{k,i}^x=\{ w \, : \, v_{k,i}^{L} \leq V_{k+1}^{*}(f^w(x,u)) < v_k^{U}  \}$ and such that for each  $k\in [0,N],$ $H_{k,i}^x \cap H_{k,j}^x $ for $i,j\in \{1,...,n_p \}$.  If $\pi^*$ is such that $V^*_0=V^{\pi^*}_0$, then $\pi^*$ is a maximal safe strategy. 
\end{theorem}
A proof for Theorem \ref{Th:Syntesis} can be derived similarly to  \cite[Theorem 2]{abate2008probabilistic}. \LL{I did not do re-do the full derivation, but everything should follow similarly. MAybe we can add a sketch.}

A numerical algorithm for computing $\pi^*$ is given in Algorithm...\LL{need to explain how you build the extended sets that are kept fixed in Theorem 2}\LL{Also }








%\LL{Sono arrivato qui. Da finire}

%To show the correctness of Algorithm \ref{alg:ForLoop} we first need to establish the following result, which is the core of our backward procedure

%\begin{proposition}
%\label{prop:CorrectnessBack}
%Let $k\in [0,T-1]$ and ${Q}^{enl}\subseteq \mathcal{G}\cup \mathcal{S}$
% \footnote{\np{not sure the prop below works for any ${Q}^{enl}$ but only for ${Q}^{enl}$  as per line 6 of the algorithm?}\LL{it holds for any $\beta(x,k)\subseteq \mathcal{G}\cup\mathcal{S}$}
%and assume, as per Problem 1, that $\mathcal{G}\cap \mathcal{S}=\emptyset$. Then, it holds that
%$$  P_{reach}(\mathcal{G},\mathcal{S},q,[k,T])\geq \inf_{x\in q} T^{}({Q}^{enl}|x)\cdot \inf_{\bar x \in \beta(x,k)} P_{reach}(\mathcal{G},\mathcal{S},\bar x,[k+1,T],\pi).$$
%\end{proposition}

%\begin{proof}
%For any $x\in q$ it holds that
%\begin{align*}
 %    &P_{reach}(\mathcal{G},\mathcal{S},x,[k,T])=\\
 %    &\sum_{j=k+1}^{T}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' < j, \omega(j') \in \mathcal{S} |\omega(k)= x)\geq\\
  %  &Pr( \omega(k+1) \in \mathcal{G} |\omega(k)= x ) +\\
  %  &\quad Pr( \omega(k+1) \in (\beta(x,k)-\mathcal{G}) |\omega(k)= x ) \sum_{j=k+2}^{T}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' < j, \omega(j') \in \mathcal{S} |\omega(k+1)\in (\beta(x,k)-\mathcal{G}))\geq\\
  %  &Pr( \omega(k+1) \in \beta(x,k) |\omega(k)= x ) \sum_{j=k+2}^{T}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' < j, \omega(j') \in \mathcal{S} |\omega(k+1)\in (\beta(x,k)-\mathcal{G}))\geq\\
  %  &Pr( \omega(k+1) \in \beta(x,k) |\omega(k)= x )\inf_{\bar x \in \beta(x,k)} \sum_{j=k+2}^{T}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' < j, \omega(j') \in \mathcal{S} |\omega(k+1)=\bar x)=\\
  %  &Pr( \omega(k+1) \in \beta(x,k) |\omega(k)= x )\inf_{\bar x \in \beta(x,k)} P_{reach}(\mathcal{G},\mathcal{S},\bar x,[k+1,T]),
%\end{align*}
%where the third passage holds because  $\sum_{j=k+2}^{T}P( \omega(j) \in \mathcal{G} \wedge \forall j' < j, \omega(j') \in \mathcal{S} |\omega(k+1)\in (\beta(x,k)-\mathcal{G}))$ is a sum of the probabilities of mutually exclusive events, hence a probability itself and by definition smaller or equal than $1$. 
%\end{proof}



%It is possible to note that Proposition \ref{prop:CorrectnessBack} is employed in line 8 of Algorithm \ref{alg:ForLoop} to extend the goal region over time with a lower bound of $P_{reach}$. We can now consider the following theorem, whose proof follows by induction applying Proposition \ref{prop:CorrectnessBack} 

%\begin{theorem}
%Let $\hat P_{\mathcal{G},\mathcal{S},[0.N]}^{\pi}$ be as computed in Algorithm \ref{alg:ForLoop}. Then, for any $x\in \mathcal{S}$ it holds that
%$$ \hat P_{\mathcal{G},\mathcal{S},[0.N]}^{\pi}(x)\leq P_{reach}(\mathcal{G},\mathcal{S},x,[0.N],\pi)$$
%\end{theorem}

==> Sections/Proofs.tex <==
\section{Proofs}

\textbf{Proof of Theorem \ref{th:CorrectnessBack}}
The proof is by induction. The base case is $k=N$, for which we have
$$V_N^{\pi}(x) \leq P_{reach}(\mathcal{G},\mathcal{S},x,[N,N]|\pi)= \mathbf{1}_\mathcal{G}(x), $$
which is trivially verified. Now with the assumption that for any $k\in \{0,N-1 \}$ it holds that 
\begin{align}
    \label{Eqn:IndBaseCase}
  V_{k+1}^{\pi}(x) \leq P_{reach}(\mathcal{G},\mathcal{S},x,[k+1,N]|\pi),
\end{align}
we can show the induction step.
In particular, for any $x$ the following holds (in the rest of the proof for simplicity we omit the dependence of the strategy from $Pr$)
\begin{align*}
     &P_{reach}(\mathcal{G},\mathcal{S},x,[k,N]|\pi)=\\
     &\sum_{j=k}^{N}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' \in [k,j) , \omega(j') \in \mathcal{S} |\omega(k)= x)= \\
     &\mathbf{1}_{\mathcal{G}}(x) + \mathbf{1}_{\mathcal{S}}(x)\sum_{j=k+1}^{N}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' \in [k,j), \omega(j') \in \mathcal{S} |\omega(k)= x)
\end{align*}     
Now in order to conclude the proof we first want to show that
$$ \sum_{j=k+1}^{N}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' \in [k,j)+1, \omega(j') \in \mathcal{S} |\omega(k)= x) = \int  P_{reach}(\mathcal{G},\mathcal{S},\bar x,[k+1,N]| \pi)T(\bar{x}|x)  d\bar{x}. $$
In order to do so, we can proceed as follow
\begin{align*}
   & \sum_{j=k+1}^{N}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' \in [k+1,j), \omega(j') \in \mathcal{S} |\omega(k)= x)=\\
 & Pr( \omega(k+1) \in \mathcal{G} |\omega(k)=x)+ \\
 &\quad \sum_{j=k+2}^{N}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' \in [k+1,j), \omega(j') \in \mathcal{S} |\omega(k+1)\in \mathcal{S},  \omega(k)= x)Pr(\omega(k+1)\in \mathcal{S} | \omega(k)= x))=\\
  & \int_{\mathcal{G}} T(\bar{x}|x) d\bar{x} + \\
 &\quad \sum_{j=k+2}^{N}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' \in [k+1,j), \omega(j') \in \mathcal{S} |\omega(k+1)\in \mathcal{S},  \omega(k)= x)Pr(\omega(k+1)\in \mathcal{S} | \omega(k)= x))=\\
   & \int_{\mathcal{G}} T(\bar{x}|x) d\bar{x} + \sum_{j=k+2}^{N}Pr( \omega(j) \in \mathcal{G} \wedge \forall j' \in [k+1,j), \omega(j') \in \mathcal{S} \wedge \omega(k+1)\in \mathcal{S} |  \omega(k)= x)=\\
  & \int_{\mathcal{G}} T(\bar{x}|x) d\bar{x} + \sum_{j=k+2}^{N}\int_{\mathcal{S}} Pr( \omega(j) \in \mathcal{G} \wedge \forall j' \in [k+1,j), \omega(j') \in \mathcal{S}   | \omega(k+1)=\bar{x} )T(\bar{x}|x) d{\bar{x}}=\\
   & \int \big( \mathbf{1}_{\mathcal{G}}(\bar{x}) + \mathbf{1}_{\mathcal{S}}(\bar{x}) \sum_{j=k+2}^{N} Pr( \omega(j) \in \mathcal{G} \wedge \forall j' \in [k+1,j), \omega(j') \in \mathcal{S}   | \omega(k+1)=\bar{x} )\big)T(\bar{x}|x) d{\bar{x}}=\\
    & \int P_{reach}(\mathcal{G},\mathcal{S},\bar x,[k+1,N]| \pi)T(\bar{x}|x) d{\bar{x}}\\
\end{align*}
where the third passage holds by application of the Bayes' rule for three events.

Finally, the proof is completed by rewriting everything in weight space
\begin{align*}
    & \int  P_{reach}(\mathcal{G},\mathcal{S},\bar x,[k+1,N]| \pi)T(\bar{x}|x)  d\bar{x}= \\
    &\int  P_{reach}(\mathcal{G},\mathcal{S},f^w(\bar{x},\pi(x,k),[k+1,N]| \pi) p(w|\mathcal{D})  dw =\\
    &\sum_{i=1}^{n_p}\int_{H_{k,i}^{\pi}}  P_{reach}(\mathcal{G},\mathcal{S},f^w(\bar{x},\pi(x,k),[k+1,N]| \pi) p(w|\mathcal{D})  dw \geq\\
    &\sum_{i=1}^{n_p}\int_{H_{k,i}^{\pi}}  v_{i-1} p(w|\mathcal{D})  dw,
\end{align*}
     where the last step holds because by assumption we know that $P_{reach}(\mathcal{G},\mathcal{S},f^w(\bar{x},\pi(x,k),[k+1,N]| \pi)\geq V_{k+1}^\pi(f^w(\bar{x},\pi(x,k))$ and by construnction of sets $H_{k,i}^{\pi}$ for each of its weights $V_{k+1}^\pi(f^w(\bar{x},\pi(x,k))$ is lowerbounded by $v_{i-1}$.
     
     
     



